Second-Order Real Nodal-Line Semimetal in Three-Dimensional Graphdiyne

Real topological phases featuring real Chern numbers and second-order boundary modes have been a focus of current research, but finding their material realization remains a challenge. Here, based on first-principles calculations and theoretical analysis, we reveal the already experimentally synthesized three-dimensional (3D) graphdiyne as the first realistic example of the recently proposed second-order real nodal-line semimetal. We show that the material hosts a pair of real nodal rings, each protected by two topological charges: a real Chern number and a 1D winding number. The two charges generate distinct topological boundary modes at distinct boundaries. The real Chern number leads to a pair of hinge Fermi arcs, whereas the winding number protects a double drumhead surface bands. We develop a low-energy model for 3D graphdiyne which captures the essential topological physics. Experimental aspects and possible topological transition to a 3D real Chern insulator phase are discussed.

==> Makefile <==
LATEX = latex 
BIBTEX = bibtex
DVIPDF = dvipdfmx
PDFLATEX = pdflatex


tex_base =SONLSM_v1221

pdf: 
	$(PDFLATEX)  $(tex_base)	
	$(BIBTEX)    $(tex_base)
	$(PDFLATEX)  $(tex_base)	
	$(PDFLATEX)  $(tex_base)	

clean :
	rm -vf $(tex_base).dvi $(tex_base).log $(tex_base).aux $(tex_base).bbl \
	$(tex_base).blg *$(tex_base).ilg $(tex_base).toc $(tex_base).lof \
	$(tex_base).lot $(tex_base).idx $(tex_base).ind $(tex_base).out \
	$(tex_base).ps figs/*.pdf



